Feedback Completion Certificates for Repeated Dwell Tasks with Time Windows

An inspection robot may owe several measurements at the same station, each with a different window in which a dwell can begin. We ask what a feedback controller must retain about earlier visits to guarantee all remaining deadlines under bounded disturbances. For a common spatial predicate and dwell length, removing redundant windows orders the remaining obligations by both endpoints. On every history without an expired obligation, the served windows form a suffix. One boundary and one capped run length therefore preserve the future satisfaction of the original task. On a verified library of branching motion primitives we use this state to recover a feedback policy. For one task type a scalar threshold per run length suffices, with work linear in the number of listed branches per time layer for fixed dwell. Multiple types require a joint recursion. On a quadrotor inspection library the threshold sweep reduced the cost of constructing a reusable full-domain policy, while a sparse Boolean baseline answered a single initial query faster. In a two-station MuJoCo patrol, three task-aware filters all met every window in twelve paired runs each. Of eight initially certified runs, the completion filter retained the certificate in all eight, compared with three for safety-only filtering.

==> proofs/00-preface.tex <==
\ifdefined\UseExternalMain
This supplement contains full proofs of the results in the main paper. Numbers
of results, definitions, assumptions, equations, algorithms, sections and
figures refer to the main paper; equations numbered (S1), (S2), \dots\ are
local to this supplement. Each result is restated before its proof.
\else
\section*{Full proofs}
This appendix contains full proofs of all results; each result is restated
before its proof. In the submission, this material forms the supplement.
\fi


==> sections/00-abstract.tex <==
We study receding-horizon control of constrained linear systems for bounded
reach--dwell--avoid tasks that must hold under a spatial error budget and
under every constant, one-sided timing offset up to a bound. On every
non-failed history the served offsets form a suffix, so one integer and one
dwell counter per task represent the completion state exactly. On a verified
transition library, a backward recursion over this state yields terminal
completion certificates, and storing only minimal winning states certifies the
same sets; with a one-sided bit encoding and a verified initial candidate,
the short-horizon controller is recursively feasible and satisfies the task
for all admissible offsets and perturbations. For a known nonlinear system
with bounded disturbances, a verified branching library lets one action reach
several regions; for each fixed tuple of successor target states, the robust
recursion has at most two predecessor candidates per task, irrespective of
the number of branches, and the certificate is a
branch feedback that completes every offset by the original deadline. In
MuJoCo quadrotor simulation, a task that provably needs two separated visits
completes in every run; online re-solving improves on the verified backup,
which carries an optimizer outage, while full-horizon replanning is better
with a longer execution window. On a declared discrete unicycle with
interval-verified primitives, the actual initial state is certified, two
admissible disturbances from it lead to branches with disjoint sets of
library-certified next actions, and two legal
histories that end at the same state and clock have disjoint certified action
sets. The robot evidence is empirical.


==> sections/01-introduction.tex <==
\section{Introduction}\label{sec:intro}

A quadrotor must dwell in an inspection region during a window of a task
clock that an operator or a supervising system starts. The start command
reaches the robot after a latency that is fixed once the task begins but
known only up to $D$ samples, so in the robot's clock the window is shifted by
an unknown $d\in\{0,\dots,D\}$, and every $d$ must be served. This is not an
input delay (the robot's own actuation is on time), not a measurement delay
(the robot knows its state), and not jitter (the shift does not change during
the task; Remark~\ref{rem:jitter}). One visit may serve only some offsets. A
controller with a short prediction horizon must retain which offsets its
executed visits have served and certify that each remaining one can still be
served before its own deadline.

The fixed-offset requirement compiles exactly into finite-horizon STL over
tightened bits (Proposition~\ref{prop:compile}), so synchronous temporal
robustness and its MILP encodings~\cite{rodionova2023tecs,yu2023atr},
history-preserving control~\cite{ilyes2025rcpe,ilyes2026rotogo} and
temporal-logic terminal constructions~\cite{yu2022decomp,vlahakis2024recurring}
already apply. We ask what the structure of reach--dwell--avoid tasks adds:
\begin{itemize}
\item \emph{Compact completion state.} Served offsets form a suffix on every
non-failed history (Theorem~\ref{thm:suffix}). One integer and one dwell counter
per task replace a $(D+1)$-bit coverage set, with exact updates and expiry
(Corollary~\ref{cor:compact}). Propositions~\ref{prop:hierarchy}--\ref{prop:strict}
characterize when shared-time, single-witness and single-continuous-visit
encodings are exact; separated visits are needed only beyond these.
\item \emph{Library certificates.} On the same whole-region verified transition
library, plain and ordered backward recursions certify identical sets
(Theorem~\ref{thm:dp-eq}). Closed-form minimal predecessors
(Lemma~\ref{lem:minpre}) yield a sound, successor-closed terminal certificate
(Theorem~\ref{thm:sound}).
\item \emph{Branching certificates.} For a known nonlinear system with
bounded disturbances, a verified branching library lets one action reach
several regions; for each fixed tuple of successor target states, the robust
AND/OR recursion has closed-form predecessors with at most two candidates per
task, irrespective of the number of branches (Proposition~\ref{prop:robpre};
the number of target tuples is not bounded by this), its plain,
explicit-bitset and ordered forms
coincide on the same library (Theorem~\ref{thm:robcert}), and the certificate
is an executable branch feedback that completes every offset by the original
deadline (Theorem~\ref{thm:robloop}).
\item \emph{An execution interface compatible with the completion order.}
Requiring that a claimed bit implies its tightened
predicate~\cite{kurtz2022fewer} and starting from a verified candidate give
recursive feasibility and all-offset closed-loop guarantees
under the stated model assumptions
(Theorems~\ref{thm:rf}--\ref{thm:closedloop}); on branching libraries the same
order makes the certificate a filter for any proposer
(Section~\ref{sec:filter}).
\end{itemize}
In MuJoCo quadrotor simulation, a task that
provably needs separated visits completes with both monitors in agreement,
and online re-solving improves on the verified backup; against full-horizon
replanning the comparison depends on the execution window. On a declared
discrete unicycle, two admissible disturbances from one state lead to
branches with disjoint sets of library-certified next actions, and two legal histories that end at the same state,
region and clock have disjoint certified action sets, so the completion
history changes the decision (Section~\ref{sec:eval-robust}). On matched
queries compact and bitset states are equally many, and our ordered recursion is slower
and saves memory only with four tasks and in one three-task setting. All robot evidence is empirical; proofs are in the supplement.


==> sections/02-related-work.tex <==
\section{Related Work}\label{sec:related}

\emph{Temporal robustness.} STL semantics~\cite{maler2004monitoring,donze2010robust}
underlie mixed-integer MPC~\cite{raman2014mpc} and robust
variants~\cite{sadraddini2015robust}. Rodionova et
al.~\cite{rodionova2021timerobust,rodionova2023tecs} define synchronous and
asynchronous temporal robustness, encode it as a MILP and maximize it; their
integer counters record for how many consecutive samples a predicate keeps
its value, i.e.\ how far a signal may be shifted. Integer counters are
therefore not our distinction. Our counter $c$ records which offsets of a
fixed-bound obligation the executed prefix has already served, is updated once
per sample (executed nominal bits in tube MPC, observed-state bits on
branching libraries), and is the state of a backward completion
recursion. Combined left and right robustness~\cite{rodionova2023leftright}
allows shifts in both directions; we fix a constant offset
$d\in[0,D]$ common to all outputs. A constant two-sided range $[-D_1,D_2]$
reduces to it exactly: with $d'=d+D_1$, the window $[a,b]$ becomes
$[a+D_1,b+D_1]$ and $D=D_1+D_2$, provided the horizon covers the later
deadline. Spatiotemporal robustness~\cite{schoen2026str} allows signed, componentwise
shifts and computes Pareto tradeoffs; we certify one fixed pair
$(\varepsilon,D)$ and do not claim membership in that region. Synthesis under
asynchronous temporal robustness~\cite{yu2023atr} already handles bounded
shifts, so fixed-offset semantics and their compilation
(Proposition~\ref{prop:compile}) are not new; our gain is the structural
representation of the served history.

\emph{History and terminal conditions.} Robustness-conserving partial
evaluation~\cite{ilyes2025rcpe} and robustness-to-go~\cite{ilyes2026rotogo}
retain history for general STL and apply to our compiled formula. On the
reach--dwell fragment with fixed offsets we give an exact state of one integer
and one dwell counter per task instead of the $(D+1)$-bit coverage. Terminal feasibility~\cite{mayne2000constrained,borrelli2017predictive},
tube MPC~\cite{mayne2005tube,mayne2006output}, and invariant
sets~\cite{blanchini1999set,kolmanovsky1998theory} are established tools.
Temporal-logic decomposition~\cite{yu2022decomp} and backward-reachability
terminal conditions~\cite{vlahakis2024recurring} are the closest constructions.
Uncertain navigation times~\cite{linard2024mitl} and context-triggered robust
MPC~\cite{kordabad2026ctrmpc} address different uncertainty models.

\emph{Nonlinear, robust and filtered temporal-logic control.} We claim none of
the following as new. STL runtime assurance~\cite{baird2023rta} filters
nominal inputs for nonlinear models with history obligations and libraries of
terminal sets; its interval-STL extension~\cite{baird2026interval} (preprint)
adds bounded uncertainty, recursive feasibility and a deadline backup for
linear systems. Online synthesis~\cite{yu2024online} and guaranteed
completion~\cite{jiang2024completion} use temporal-logic trees and
reachability for disturbed nonlinear systems, the latter with online
admissible input sets; value functions~\cite{so2026value} separate completion
from satisfiability with history-dependent policies and filters. In these
frameworks, our state replaces the history obligation of the fragment, and its
suffix structure makes each robust predecessor step closed form on a verified
branching library; we add no new filter architecture. Reduced
STL encodings~\cite{kurtz2022fewer} motivate our one-directional bit
implications, and minimal-element representations are standard in
synthesis~\cite{dewulf2006antichains,cadilhac2022acacia}.


==> sections/08-limitations.tex <==
\section{Limitations and Conclusion}\label{sec:limits}

The results cover constant synchronous one-sided offsets, one fixed
$(\varepsilon,D)$ and the positive reach--dwell--avoid fragment, without a
robustness frontier, general STL, delays or jitter. Compact states are
exponential in task count and target vectors per branching edge unbounded;
initialization needs a timely verified candidate. Guarantees concern the
declared models and hold on the robot only while the measured residual stays in
$\mathcal W$, as it did in every run. The short
horizon was not faster than a full-horizon encoding and beat full-horizon
replanning only in one setting.
Certificates are exact only relative to one abstraction, the single-successor
obstruction is limited to position-independent primitives on product boxes,
and the filter mattered only in targeted cases.

